The case of the missing VHE GRBs: A retrospective study of Swift gamma-ray bursts with Imaging Atmospheric Cherenkov Telescopes

Gamma-ray bursts (GRBs) are particle acceleration sites that can emit photons in the very high-energy (VHE) domain through non-thermal processes. From 2004 until 2018, the current generation of Imaging Atmospheric Cherenkov Telescopes (IACTs) did not detect any GRB in the VHE domain. However, from 2018 to 2020, five detections have been reported. In this work, we try to solve the case of the missing VHE GBRs prior to 2018. We aim to identify GRBs that might have eluded VHE detection in the past years by the H.E.S.S., MAGIC, and VERITAS IACTs. To do so, we study GRBs with known redshift detected by \emph{Swift} from 2004 until June 2022. We first identify all GRBs that could have been observed by these IACTs since 2004, considering observation conditions and visibility constraints. We assume a relation between the X-rays and the VHE gamma rays based on the VHE GRBs detected to date and combine this with the redshift measurements, instrument response information, and observation conditions to predict the observed VHE gamma-ray flux from the \emph{Swift}-XRT measurements. We report findings on 12 bright low-redshift GRBs that we identify as most likely to have been detected in the VHE domain by current IACTs. The rate of IACT-detectable GRBs with ideal observation conditions is $<$1 VHE GRB per year with the current configuration. With its lower energy threshold and higher sensitivity, this rate increases to $\sim$4 VHE GRBs per year with CTA.

==> Tables/CTAS_RES5_LATEX <==
\begin{table}
\begin{tabular}{cccccccccc}
ID & GRB Name & Redshift & Burst time & Obs. delay & Obs. duration & ON & OFF & ALPHA & SIG \\
1013243 & GRB201216C & 1.1 & 2020-12-16T23:07:31.000 & 5868.999999999994 & 8131.000000000002 & 1187.962737780066 & 3780.5535484276284 & 0.2 & 13.034319140249034 \\
220020 & GRB060719 & 1.532 & 2006-07-19T06:50:36.000 & 9.000000000001407 & 12137.000000000002 & 1364.679757771807 & 5643.1654676258995 & 0.2 & 6.173515616378709 \\
305288 & GRB080310 & 2.42743 & 2008-03-10T08:37:58.000 & 33.99999999999732 & 3267.0000000000023 & 471.7497831498181 & 1519.00977034966 & 0.2 & 8.018296705979164 \\
308041 & GRB080330 & 1.5119 & 2008-03-30T03:41:16.000 & 28.99999999999814 & 1705.0000000000043 & 471.7497831498181 & 1519.00977034966 & 0.2 & 8.018296705979164 \\
309111 & GRB080413B & 1.1014 & 2008-04-13T08:51:12.000 & 29.999999999999893 & 3363.0000000000027 & 741.1093542999641 & 1563.6455028117257 & 0.2 & 18.1936251744616 \\
312958 & GRB080602 & 1.8204 & 2008-06-02T01:30:28.000 & 27648.0 & 2424.0 & 741.1093542999641 & 1563.6455028117257 & 0.2 & 18.1936251744616 \\
316534 & GRB080710 & 0.8454 & 2008-07-10T07:13:10.000 & 52.999999999997094 & 10788.000000000004 & 1686.4677972130567 & 5015.940435424587 & 0.2 & 17.6277442330344 \\
330856 & GRB081007 & 0.5295 & 2008-10-07T05:23:52.000 & 220.99999999999937 & 5477.999999999998 & 960.9045388789393 & 2547.026483616599 & 0.2 & 15.906179781937373 \\
424733 & GRB100615A & 1.398 & 2010-06-15T01:59:03.000 & 28.00000000000118 & 4685.000000000006 & 939.9959464155695 & 2178.3167352580804 & 0.2 & 18.58685791292696 \\
425151 & GRB100621A & 0.542 & 2010-06-21T03:03:32.000 & 13555.0 & 12120.0 & 1721.2311815933606 & 5635.261223335741 & 0.2 & 14.783626321246299 \\
426114 & GRB100628A & 0.102 & 2010-06-28T08:16:40.000 & 53993.0 & 3029.9999999999986 & 1721.2311815933606 & 5635.261223335741 & 0.2 & 14.783626321246299 \\
431605 & GRB100814A & 1.44 & 2010-08-14T03:50:11.000 & 2006.0000000000002 & 20142.000000000007 & 2176.155255262916 & 9365.134617197073 & 0.2 & 6.205079269734583 \\
512035 & GRB120119A & 1.728 & 2012-01-19T04:04:30.000 & 29.999999999995097 & 8145.000000000002 & 2348.0153042361057 & 3787.062926078352 & 0.2 & 40.38277655733459 \\
533060 & GRB120909A & 3.93 & 2012-09-09T01:42:03.000 & 41.000000000000014 & 10619.000000000004 & 1216.1150161187106 & 4937.362948069493 & 0.2 & 6.368558009748644 \\
536831 & GRB121027A & 1.773 & 2012-10-27T07:32:29.000 & 3249.000000000004 & 1176.9999999999986 & 1541.4815193203542 & 547.2526782067789 & 0.2 & 57.62680266871997 \\
542441 & GRB121217A & 3.1 & 2012-12-17T07:17:47.000 & 37.999999999999545 & 4276.000000000004 & 645.7292458671728 & 1988.1499167478257 & 0.2 & 10.24824227455594 \\
554620 & GRB130427A & 0.3399 & 2013-04-27T07:47:57.000 & 57691.0 & 606.0000000000132 & 110.74484339737718 & 281.7630611667938 & 0.2 & 5.704276527215984 \\
571830 & GRB130925A & 0.348 & 2013-09-25T04:11:24.000 & 80871.0 & 5606.000000000002 & 1929.0271973394533 & 2606.5407935660205 & 0.2 & 40.95260246540627 \\
652847 & GRB150821A & 0.755 & 2015-08-21T09:44:00.000 & 181.0000000000011 & 503.99999999999727 & 326.35058302066113 & 234.33759542584144 & 0.2 & 22.19961125565935 \\
727541 & GRB161219B & 0.1475 & 2016-12-19T18:48:39.000 & 21572.000000000007 & 12119.999999999995 & 1870.7619380238314 & 5635.261223335741 & 0.2 & 18.15524123188815 \\
848890 & GRB180720B & 0.654 & 2018-07-20T14:21:44.000 & 56873.99999999999 & 14545.000000000002 & 1790.8826841855337 & 6762.778423549372 & 0.2 & 10.272934134674284 \\
866434 & GRB181010A & 1.39 & 2018-10-10T05:55:51.000 & 32.999999999995566 & 11155.0 & 1450.6098339578116 & 5186.579120982688 & 0.2 & 10.930351563589584 \\
922968 & GRB190829A & 0.0785 & 2019-08-29T19:56:44.000 & 32934.99999999999 & 16817.0 & 4821.969286082938 & 7819.157425151579 & 0.2 & 57.653601664015916 \\
\end{tabular}
\end{table}

